Adaptive Discrete Smoothing for High-Dimensional and Nonlinear Panel Data

In this paper we develop a data-driven smoothing technique for high-dimensional and non-linear panel data models. We allow for individual specific (non-linear) functions and estimation with econometric or machine learning methods by using weighted observations from other individuals. The weights are determined by a data-driven way and depend on the similarity between the corresponding functions and are measured based on initial estimates. The key feature of such a procedure is that it clusters individuals based on the distance / similarity between them, estimated in a first stage. Our estimation method can be combined with various statistical estimation procedures, in particular modern machine learning methods which are in particular fruitful in the high-dimensional case and with complex, heterogeneous data. The approach can be interpreted as a \textquotedblleft soft-clustering\textquotedblright\ in comparison to traditional\textquotedblleft\ hard clustering\textquotedblright that assigns each individual to exactly one group. We conduct a simulation study which shows that the prediction can be greatly improved by using our estimator. Finally, we analyze a big data set from didichuxing.com, a leading company in transportation industry, to analyze and predict the gap between supply and demand based on a large set of covariates. Our estimator clearly performs much better in out-of-sample prediction compared to existing linear panel data estimators.

==> sim_lasso.tex <==
\subsection{Lasso Setting}


\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Lasso - out of sample - Setting 1, X iid,
p=15, s=5}\tabularnewline
\toprule
N & T & cor & MSELASSO & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & cor & MSELASSO & MSEDS\tabularnewline
\midrule
\endhead
10 & 5 & 0 & 9807.7227 & 9394.1056\tabularnewline
10 & 5 & 0.5 & 7125.8460 & 697.8030\tabularnewline
10 & 5 & 1 & 29322.5048 & 728.9525\tabularnewline
50 & 5 & 0 & 27214.9658 & 1183.4467\tabularnewline
50 & 5 & 0.5 & 21961.9780 & 2561.5256\tabularnewline
50 & 5 & 1 & 15798.8101 & 362.8937\tabularnewline
100 & 5 & 0 & 24774.7869 & 4383.5948\tabularnewline
100 & 5 & 0.5 & 9115.0330 & 1201.6366\tabularnewline
100 & 5 & 1 & 17421.0693 & 1404.9360\tabularnewline
10 & 10 & 0 & 6.5757 & 5.5606\tabularnewline
10 & 10 & 0.5 & 4.8400 & 2.5980\tabularnewline
10 & 10 & 1 & 5.4107 & 1.6479\tabularnewline
50 & 10 & 0 & 10.3866 & 9.6920\tabularnewline
50 & 10 & 0.5 & 10.9481 & 8.6209\tabularnewline
50 & 10 & 1 & 5.6059 & 1.2032\tabularnewline
100 & 10 & 0 & 25.9182 & 25.4916\tabularnewline
100 & 10 & 0.5 & 41.2791 & 39.7993\tabularnewline
100 & 10 & 1 & 10.2785 & 5.8618\tabularnewline
10 & 25 & 0 & 1.4707 & 1.5144\tabularnewline
10 & 25 & 0.5 & 1.3978 & 1.0465\tabularnewline
10 & 25 & 1 & 1.4948 & 0.0687\tabularnewline
50 & 25 & 0 & 1.4107 & 2.3890\tabularnewline
50 & 25 & 0.5 & 1.4153 & 1.5704\tabularnewline
50 & 25 & 1 & 1.4239 & 0.0114\tabularnewline
100 & 25 & 0 & 1.4205 & 2.8330\tabularnewline
100 & 25 & 0.5 & 1.3933 & 1.8057\tabularnewline
100 & 25 & 1 & 1.3840 & 0.0055\tabularnewline
10 & 50 & 0 & 0.5047 & 0.6573\tabularnewline
10 & 50 & 0.5 & 0.4862 & 0.6352\tabularnewline
10 & 50 & 1 & 0.4678 & 0.0232\tabularnewline
50 & 50 & 0 & 0.4920 & 1.6252\tabularnewline
50 & 50 & 0.5 & 0.4924 & 1.3506\tabularnewline
50 & 50 & 1 & 0.4595 & 0.0039\tabularnewline
100 & 50 & 0 & 0.4951 & 2.1594\tabularnewline
100 & 50 & 0.5 & 0.4879 & 1.6079\tabularnewline
100 & 50 & 1 & 0.5212 & 0.0021\tabularnewline
\bottomrule
\end{longtable}

%\begin{longtable}[]{@{}lllll@{}}
%\caption{Simulation Results Lasso - out of sample - Setting 1, X iid,
%p=15, s=5, c=4}\tabularnewline
%\toprule
%N & T & cor & MSELASSO & MSEDS\tabularnewline
%\midrule
%\endfirsthead
%\toprule
%N & T & cor & MSELASSO & MSEDS\tabularnewline
%\midrule
%\endhead
%%10 & 5 & 0 & 9807.7227 & 33013.8121\tabularnewline
%%10 & 5 & 0.5 & 7125.8460 & 1663.4461\tabularnewline
%%10 & 5 & 1 & 29322.5048 & 1785.6391\tabularnewline
%%50 & 5 & 0 & 27214.9658 & 3420.6666\tabularnewline
%%50 & 5 & 0.5 & 21961.9780 & 6633.2010\tabularnewline
%%50 & 5 & 1 & 15798.8101 & 2945.0271\tabularnewline
%100 & 5 & 0 & 24774.7869 & 5952.9528\tabularnewline
%100 & 5 & 0.5 & 9115.0330 & 2151.1595\tabularnewline
%100 & 5 & 1 & 17421.0693 & 3211.7221\tabularnewline
%10 & 10 & 0 & 6.5757 & 9.0366\tabularnewline
%10 & 10 & 0.5 & 4.8400 & 6.2791\tabularnewline
%10 & 10 & 1 & 5.4107 & 5.5987\tabularnewline
%50 & 10 & 0 & 10.3866 & 14.3400\tabularnewline
%50 & 10 & 0.5 & 10.9481 & 14.8347\tabularnewline
%50 & 10 & 1 & 5.6059 & 7.4526\tabularnewline
%100 & 10 & 0 & 25.9182 & 28.9459\tabularnewline
%100 & 10 & 0.5 & 41.2791 & 45.8052\tabularnewline
%100 & 10 & 1 & 10.2785 & 11.5478\tabularnewline
%10 & 25 & 0 & 1.4707 & 0.9397\tabularnewline
%10 & 25 & 0.5 & 1.3978 & 0.8666\tabularnewline
%10 & 25 & 1 & 1.4948 & 0.4980\tabularnewline
%50 & 25 & 0 & 1.4107 & 1.2657\tabularnewline
%50 & 25 & 0.5 & 1.4153 & 1.0331\tabularnewline
%50 & 25 & 1 & 1.4239 & 0.2414\tabularnewline
%100 & 25 & 0 & 1.4205 & 1.3078\tabularnewline
%100 & 25 & 0.5 & 1.3933 & 1.0116\tabularnewline
%100 & 25 & 1 & 1.3840 & 0.1493\tabularnewline
%\bottomrule
%\end{longtable} 

\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Lasso - out of sample - Setting 1, X cor,
p=15, s=5}\tabularnewline
\toprule
N & T & cor & MSELASSO & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & cor & MSELASSO & MSEDS\tabularnewline
\midrule
\endhead
%10 & 5 & 0 & 29638.1197 & 586.7126\tabularnewline
%10 & 5 & 0.5 & 60902.4034 & 352.5303\tabularnewline
%10 & 5 & 1 & 13397.9336 & 2780.7605\tabularnewline
%50 & 5 & 0 & 15205.8861 & 734.6533\tabularnewline
%50 & 5 & 0.5 & 23586.6180 & 770.1953\tabularnewline
%50 & 5 & 1 & 28475.7771 & 2722.8689\tabularnewline
%100 & 5 & 0 & 56634.3853 & 1095.8141\tabularnewline
%100 & 5 & 0.5 & 29962.2438 & 1209.3545\tabularnewline
%100 & 5 & 1 & 28244.3757 & 1231.3771\tabularnewline
10 & 10 & 0 & 3.5783 & 3.1561\tabularnewline
10 & 10 & 0.5 & 3.7155 & 2.3549\tabularnewline
10 & 10 & 1 & 5.0942 & 1.8677\tabularnewline
50 & 10 & 0 & 11.2201 & 11.0931\tabularnewline
50 & 10 & 0.5 & 4.4456 & 2.9577\tabularnewline
50 & 10 & 1 & 3.9552 & 0.2987\tabularnewline
100 & 10 & 0 & 5.6099 & 5.8097\tabularnewline
100 & 10 & 0.5 & 4.5854 & 3.1772\tabularnewline
100 & 10 & 1 & 16.2045 & 12.8038\tabularnewline
10 & 25 & 0 & 1.3949 & 1.5799\tabularnewline
10 & 25 & 0.5 & 1.3634 & 1.1555\tabularnewline
10 & 25 & 1 & 1.4258 & 0.1219\tabularnewline
50 & 25 & 0 & 1.3604 & 2.4301\tabularnewline
50 & 25 & 0.5 & 1.3976 & 1.6055\tabularnewline
50 & 25 & 1 & 1.3339 & 0.0150\tabularnewline
%100 & 25 & 0 & 1.3944 & 2.9070\tabularnewline
%100 & 25 & 0.5 & 1.3499 & 1.7905\tabularnewline
%100 & 25 & 1 & 1.3184 & 0.0079\tabularnewline
%10 & 50 & 0 & 0.6541 & 0.8595\tabularnewline
%10 & 50 & 0.5 & 0.6403 & 0.7694\tabularnewline
%10 & 50 & 1 & 0.6099 & 0.0407\tabularnewline
%50 & 50 & 0 & 0.6430 & 1.8651\tabularnewline
%50 & 50 & 0.5 & 0.6494 & 1.4133\tabularnewline
%50 & 50 & 1 & 0.5710 & 0.0064\tabularnewline
%100 & 50 & 0 & 0.6376 & 2.3625\tabularnewline
%100 & 50 & 0.5 & 0.6496 & 1.6408\tabularnewline
%100 & 50 & 1 & 0.6619 & 0.0030\tabularnewline
\bottomrule
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Lasso - out of sample - Setting 2, X iid,
p=15, s=5}\tabularnewline
\toprule
& N & T & MSELASSO & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
& N & T & MSELASSO & MSEDS\tabularnewline
\midrule
\endhead
1 & 2 & 10 & 6.5041 & 4.9281\tabularnewline
2 & 5 & 10 & 6.8800 & 2.6220\tabularnewline
3 & 10 & 10 & 6.8314 & 1.0121\tabularnewline
4 & 2 & 20 & 2.9264 & 1.5121\tabularnewline
5 & 5 & 20 & 3.0506 & 0.4947\tabularnewline
6 & 10 & 20 & 2.9579 & 0.2814\tabularnewline
7 & 2 & 50 & 0.3853 & 0.1905\tabularnewline
8 & 5 & 50 & 0.3577 & 0.1351\tabularnewline
9 & 10 & 50 & 0.3592 & 0.1422\tabularnewline
10 & 2 & 100 & 0.1022 & 0.0877\tabularnewline
11 & 5 & 100 & 0.1066 & 0.1065\tabularnewline
12 & 10 & 100 & 0.1043 & 0.1296\tabularnewline
13 & 50 & 10 & 6.8359 & 0.3740\tabularnewline
21 & 50 & 20 & 2.9423 & 0.2257\tabularnewline
31 & 50 & 50 & 0.3782 & 0.1684\tabularnewline
41 & 50 & 100 & 0.1036 & 0.1494\tabularnewline
\bottomrule
\end{longtable}

\begin{longtable}[]{@{}llll@{}}
\caption{Simulation Results Lasso - out of sample - Setting 2, X cor,
p=15, s=5}\tabularnewline
\toprule
N & T & MSELASSO & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & MSELASSO & MSEDS\tabularnewline
\midrule
\endhead
2 & 10 & 5.7229 & 4.1633\tabularnewline
5 & 10 & 5.7531 & 1.7605\tabularnewline
10 & 10 & 5.5935 & 0.7353\tabularnewline
50 & 10 & 5.5829 & 0.2970\tabularnewline
2 & 20 & 1.6070 & 0.7536\tabularnewline
5 & 20 & 1.5618 & 0.2914\tabularnewline
10 & 20 & 1.5467 & 0.2080\tabularnewline
50 & 20 & 1.5342 & 0.1651\tabularnewline
2 & 50 & 0.1816 & 0.1330\tabularnewline
5 & 50 & 0.1751 & 0.1111\tabularnewline
10 & 50 & 0.1771 & 0.1174\tabularnewline
50 & 50 & 0.1777 & 0.1288\tabularnewline
2 & 10 & 9.5297 & 6.8394\tabularnewline
5 & 10 & 9.4982 & 1.8809\tabularnewline
10 & 10 & 9.6549 & 0.6875\tabularnewline
2 & 20 & 2.8704 & 1.4549\tabularnewline
5 & 20 & 2.9941 & 0.5697\tabularnewline
10 & 20 & 2.8249 & 0.3392\tabularnewline
2 & 50 & 0.2367 & 0.1524\tabularnewline
5 & 50 & 0.2369 & 0.1184\tabularnewline
10 & 50 & 0.2415 & 0.1165\tabularnewline
50 & 50 & 0.2389 & 0.1321\tabularnewline
50 & 100 & 0.0783 & 0.1186\tabularnewline

%2 & 100 & 0.0710 & 0.0685\tabularnewline
%5 & 100 & 0.0708 & 0.0887\tabularnewline
%10 & 100 & 0.0711 & 0.1015\tabularnewline
%50 & 100 & 0.0714 & 0.1180\tabularnewline
\bottomrule
\end{longtable}


==> sim_lasso_mod.tex <==
\subsection{Lasso Setting}

\begin{longtable}[htp]{@{}lllllll@{}}
	\caption{Simulation Results Lasso - out of sample - Setting 1, 
		p=15, s=5}\tabularnewline
	\toprule
	  &   &     & \multicolumn{2}{l}{X iid} & \multicolumn {2}{l}{X cor}  \tabularnewline
	N & T & cor & MSEOLS & MSEDS          & MSEOLS & MSEDS \tabularnewline
	\midrule
	\endfirsthead
	\toprule
	  &   &     & \multicolumn{2}{l}{X iid} & \multicolumn {2}{l}{X cor}  \tabularnewline
	N & T & cor & MSEOLS & MSEDS          & MSEOLS & MSEDS \tabularnewline
	\midrule
	\endhead
	%10 & 5 & 0 & 9807.7227 & 9394.1056\tabularnewline
	%10 & 5 & 0.5 & 7125.8460 & 697.8030\tabularnewline
	%10 & 5 & 1 & 29322.5048 & 728.9525\tabularnewline
	%50 & 5 & 0 & 27214.9658 & 1183.4467\tabularnewline
	%50 & 5 & 0.5 & 21961.9780 & 2561.5256\tabularnewline
	%50 & 5 & 1 & 15798.8101 & 362.8937\tabularnewline
	%100 & 5 & 0 & 24774.7869 & 4383.5948\tabularnewline
	%100 & 5 & 0.5 & 9115.0330 & 1201.6366\tabularnewline
	%100 & 5 & 1 & 17421.0693 & 1404.9360\tabularnewline
	10 & 10 & 0 & 6.5757 & 5.5606& 3.5783 & 3.1561\tabularnewline
	10 & 10 & 0.5 & 4.8400 & 2.5980& 3.7155 & 2.3549\tabularnewline
	10 & 10 & 1 & 5.4107 & 1.6479 & 5.0942 & 1.8677\tabularnewline
	50 & 10 & 0 & 10.3866 & 9.6920& 11.2201 & 11.0931\tabularnewline
	50 & 10 & 0.5 & 10.9481 & 8.6209 & 4.4456 & 2.9577\tabularnewline
	50 & 10 & 1 & 5.6059 & 1.2032& 3.9552 & 0.2987\tabularnewline
	100 & 10 & 0 & 25.9182 & 25.4916& 5.6099 & 5.8097\tabularnewline
	100 & 10 & 0.5 & 41.2791 & 39.7993 & 4.5854 & 3.1772\tabularnewline
	100 & 10 & 1 & 10.2785 & 5.8618& 16.2045 & 12.8038\tabularnewline
	10 & 25 & 0 & 1.4707 & 1.5144& 1.3949 & 1.5799\tabularnewline
	10 & 25 & 0.5 & 1.3978 & 1.0465& 1.3634 & 1.1555\tabularnewline
	10 & 25 & 1 & 1.4948 & 0.0687& 1.4258 & 0.1219\tabularnewline
	50 & 25 & 0 & 1.4107 & 2.3890& 1.3604 & 2.4301\tabularnewline
	50 & 25 & 0.5 & 1.4153 & 1.5704& 1.3976 & 1.6055\tabularnewline
	50 & 25 & 1 & 1.4239 & 0.0114 & 1.3339 & 0.0150\tabularnewline
	\midrule
	100 & 25 & 0 & 1.4205 & 2.8330& 1.3944 & 2.9070\tabularnewline
	100 & 25 & 0.5 & 1.3933 & 1.8057& 1.3499 & 1.7905\tabularnewline
	100 & 25 & 1 & 1.3840 & 0.0055& 1.3184 & 0.0079\tabularnewline
	10 & 50 & 0 & 0.5047 & 0.6573& 0.6541 & 0.8595\tabularnewline
	10 & 50 & 0.5 & 0.4862 & 0.6352& 0.6403 & 0.7694\tabularnewline
	10 & 50 & 1 & 0.4678 & 0.0232& 0.6099 & 0.0407\tabularnewline
	50 & 50 & 0 & 0.4920 & 1.6252& 0.6430 & 1.8651\tabularnewline
	50 & 50 & 0.5 & 0.4924 & 1.3506& 0.6494 & 1.4133\tabularnewline
	50 & 50 & 1 & 0.4595 & 0.0039& 0.5710 & 0.0064\tabularnewline
	100 & 50 & 0 & 0.4951 & 2.1594& 0.6376 & 2.3625\tabularnewline
	100 & 50 & 0.5 & 0.4879 & 1.6079  & 0.6496 & 1.6408\tabularnewline
	100 & 50 & 1 & 0.5212 & 0.0021& 0.6619 & 0.0030\tabularnewline
	\bottomrule
\end{longtable}

\begin{longtable}[]{@{}llllll@{}}
	\caption{Simulation Results Lasso - out of sample - Setting 2, p=15, s=5}\tabularnewline
	\toprule
	  &   & \multicolumn{2}{l}{X iid} & \multicolumn {2}{l}{X cor}  \tabularnewline
	N & T & MSEOLS & MSEDS          & MSEOLS & MSEDS \tabularnewline
	\midrule
	\endfirsthead
	\toprule
	  &   & \multicolumn{2}{l}{X iid} & \multicolumn {2}{l}{X cor}  \tabularnewline
	N & T & MSEOLS & MSEDS          & MSEOLS & MSEDS \tabularnewline
	\midrule
	\endhead
	 2 & 10 & 6.5041 & 4.9281 & 5.7229 & 4.1633\tabularnewline
	 5 & 10 & 6.8800 & 2.6220& 5.7531 & 1.7605\tabularnewline
	 10 & 10 & 6.8314 & 1.0121 & 5.5935 & 0.7353\tabularnewline
	 50 & 10 && & 5.5829 & 0.2970\tabularnewline
	 2 & 20 & 2.9264 & 1.5121  & 1.6070 & 0.7536\tabularnewline
	 5 & 20 & 3.0506 & 0.4947& 1.5618 & 0.2914\tabularnewline
	 10 & 20 & 2.9579 & 0.2814& 1.5467 & 0.2080\tabularnewline
	 50 & 20 && & 1.5342 & 0.1651\tabularnewline
	 2 & 50 & 0.3853 & 0.1905 & 0.1816 & 0.1330\tabularnewline
	 5 & 50 & 0.3577 & 0.1351& 0.1751 & 0.1111\tabularnewline
	 10 & 50 & 0.3592 & 0.1422 & 0.1771 & 0.1174\tabularnewline
	 50 & 50 && & 0.1777 & 0.1288\tabularnewline
	 2 & 100 & 0.1022 & 0.0877&  & \tabularnewline
	 5 & 100 & 0.1066 & 0.1065&  & \tabularnewline
	 10 & 100 & 0.1043 & 0.1296 &  & \tabularnewline
	 50 & 10 & 6.8359 & 0.3740&  & \tabularnewline
	 50 & 20 & 2.9423 & 0.2257 &  & \tabularnewline
	 50 & 50 & 0.3782 & 0.1684 & 0.2389 & 0.1321\tabularnewline
	 50 & 100 & 0.1036 & 0.1494 & 0.0783 & 0.1186\tabularnewline
	 \hline
	 2 & 10 && & 9.5297 & 6.8394\tabularnewline
	 5 & 10 && & 9.4982 & 1.8809\tabularnewline
	 10 & 10 && & 9.6549 & 0.6875\tabularnewline
	 2 & 20 && & 2.8704 & 1.4549\tabularnewline
	 5 & 20 && & 2.9941 & 0.5697\tabularnewline
	 10 & 20 && & 2.8249 & 0.3392\tabularnewline
	 2 & 50 && & 0.2367 & 0.1524\tabularnewline
	 5 & 50 && & 0.2369 & 0.1184\tabularnewline
	 10 & 50 && & 0.2415 & 0.1165\tabularnewline
	 50 & 50 && & 0.2389 & 0.1321\tabularnewline
	 50 & 100 && & 0.0783 & 0.1186\tabularnewline
	\bottomrule
\end{longtable}



==> sim_reg.tex <==
\subsection{Regression Setting}

\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Linear - out of sample - Setting 1, X iid,
p=5}\tabularnewline
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endhead
2 & 10 & 0 & 2.0477 & 1.8037\tabularnewline
2 & 10 & 0.3 & 1.8083 & 1.5804\tabularnewline
2 & 10 & 0.7 & 1.8056 & 1.3903\tabularnewline
2 & 10 & 1 & 2.0681 & 1.1047\tabularnewline
10 & 10 & 0 & 1.8735 & 1.3439\tabularnewline
10 & 10 & 0.3 & 1.8975 & 1.2038\tabularnewline
10 & 10 & 0.7 & 1.8734 & 0.8594\tabularnewline
10 & 10 & 1 & 1.9841 & 0.2563\tabularnewline
50 & 10 & 0 & 1.9364 & 1.6732\tabularnewline
50 & 10 & 0.3 & 1.8925 & 1.5160\tabularnewline
50 & 10 & 0.7 & 1.9256 & 0.9738\tabularnewline
50 & 10 & 1 & 1.8750 & 0.0557\tabularnewline
2 & 20 & 0 & 0.4585 & 0.4601\tabularnewline
2 & 20 & 0.3 & 0.4429 & 0.4380\tabularnewline
2 & 20 & 0.7 & 0.4405 & 0.4027\tabularnewline
2 & 20 & 1 & 0.4509 & 0.2285\tabularnewline
10 & 20 & 0 & 0.4501 & 0.6132\tabularnewline
10 & 20 & 0.3 & 0.4505 & 0.6299\tabularnewline
10 & 20 & 0.7 & 0.4605 & 0.5729\tabularnewline
10 & 20 & 1 & 0.4546 & 0.0444\tabularnewline
\bottomrule
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Linear - out of sample - Setting 1, X iid,
p=10}\tabularnewline
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endhead
2 & 20 & 0 & 1.4150 & 1.3666\tabularnewline
2 & 20 & 0.3 & 1.3444 & 1.2612\tabularnewline
2 & 20 & 0.7 & 1.3695 & 1.1300\tabularnewline
2 & 20 & 1 & 1.3662 & 0.6643\tabularnewline
10 & 20 & 0 & 1.3668 & 1.1860\tabularnewline
10 & 20 & 0.3 & 1.3642 & 1.1461\tabularnewline
10 & 20 & 0.7 & 1.3681 & 0.9733\tabularnewline
10 & 20 & 1 & 1.3442 & 0.1208\tabularnewline
50 & 20 & 0 & 1.3651 & 1.6518\tabularnewline
50 & 20 & 0.3 & 1.3691 & 1.7681\tabularnewline
50 & 20 & 0.7 & 1.3730 & 1.4962\tabularnewline
50 & 20 & 1 & 1.3598 & 0.0211\tabularnewline
2 & 50 & 0 & 0.2896 & 0.2901\tabularnewline
2 & 50 & 0.3 & 0.2890 & 0.2890\tabularnewline
2 & 50 & 0.7 & 0.2942 & 0.3010\tabularnewline
2 & 50 & 1 & 0.2805 & 0.1429\tabularnewline
10 & 50 & 0 & 0.2907 & 0.3431\tabularnewline
10 & 50 & 0.3 & 0.2888 & 0.4161\tabularnewline
10 & 50 & 0.7 & 0.2856 & 0.5958\tabularnewline
10 & 50 & 1 & 0.2868 & 0.0270\tabularnewline
\bottomrule
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\caption{Simulation Results Linear - out of sample - Setting 1, X cor,
p=5}\tabularnewline
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & cor & MSEOLS & MSEDS\tabularnewline
\midrule
\endhead
2 & 10 & 0 & 1.8411 & 1.6828\tabularnewline
2 & 10 & 0.3 & 1.9002 & 1.6448\tabularnewline
2 & 10 & 0.5 & 1.9717 & 1.6382\tabularnewline
2 & 10 & 0.8 & 1.9106 & 1.4015\tabularnewline
2 & 10 & 1 & 1.9148 & 1.1648\tabularnewline
10 & 10 & 0 & 1.9718 & 1.4550\tabularnewline
10 & 10 & 0.3 & 1.9239 & 1.2699\tabularnewline
10 & 10 & 0.5 & 1.9413 & 1.1295\tabularnewline
10 & 10 & 0.8 & 2.1294 & 0.9679\tabularnewline
10 & 10 & 1 & 1.9357 & 0.3262\tabularnewline
50 & 10 & 0 & 1.9365 & 1.6522\tabularnewline
50 & 10 & 0.3 & 1.9011 & 1.4880\tabularnewline
50 & 10 & 0.5 & 1.9335 & 1.2989\tabularnewline
50 & 10 & 0.8 & 1.8970 & 0.7490\tabularnewline
50 & 10 & 1 & 1.8919 & 0.0782\tabularnewline
100 & 10 & 0 & 1.9235 & 1.9808\tabularnewline
100 & 10 & 0.3 & 1.9332 & 1.7589\tabularnewline
100 & 10 & 0.5 & 1.9416 & 1.4893\tabularnewline
100 & 10 & 0.8 & 1.9211 & 0.8225\tabularnewline
100 & 10 & 1 & 1.8920 & 0.0485\tabularnewline
2 & 20 & 0 & 0.4459 & 0.4596\tabularnewline
2 & 20 & 0.3 & 0.4490 & 0.4546\tabularnewline
2 & 20 & 0.5 & 0.4526 & 0.4351\tabularnewline
2 & 20 & 0.8 & 0.4789 & 0.4131\tabularnewline
2 & 20 & 1 & 0.4717 & 0.2574\tabularnewline
%10 & 20 & 0 & 0.4508 & 0.5969\tabularnewline
%10 & 20 & 0.3 & 0.4466 & 0.6316\tabularnewline
%10 & 20 & 0.5 & 0.4610 & 0.6230\tabularnewline
%10 & 20 & 0.8 & 0.4475 & 0.4702\tabularnewline
%10 & 20 & 1 & 0.4500 & 0.0497\tabularnewline
\bottomrule
\end{longtable}

\begin{longtable}[]{@{}llll@{}}
\caption{Simulation Results Linear - out of sample - Setting 2, X iid,
p=5}\tabularnewline
\toprule
N & T & MSEOLS & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & MSEOLS & MSEDS\tabularnewline
\midrule
\endhead
2 & 10 & 1.7442 & 1.1173\tabularnewline
5 & 10 & 1.9357 & 0.6869\tabularnewline
10 & 10 & 1.9140 & 0.4323\tabularnewline
50 & 10 & 1.9496 & 0.2680\tabularnewline
100 & 10 & 1.9326 & 0.2364\tabularnewline
2 & 20 & 0.4488 & 0.3057\tabularnewline
5 & 20 & 0.4558 & 0.1996\tabularnewline
10 & 20 & 0.4630 & 0.1653\tabularnewline
50 & 20 & 0.4520 & 0.1561\tabularnewline
100 & 20 & 0.4544 & 0.1586\tabularnewline
2 & 50 & 0.1416 & 0.1155\tabularnewline
5 & 50 & 0.1402 & 0.1071\tabularnewline
10 & 50 & 0.1411 & 0.1160\tabularnewline
50 & 50 & 0.1375 & 0.1298\tabularnewline
100 & 50 & 0.1381 & 0.1336\tabularnewline
2 & 100 & 0.0640 & 0.0663\tabularnewline
\bottomrule
\end{longtable}


\begin{longtable}[]{@{}llll@{}}
\caption{Simulation Results Linear - out of sample - Setting 2, X cor,
p=5}\tabularnewline
\toprule
N & T & MSEOLS & MSEDS\tabularnewline
\midrule
\endfirsthead
\toprule
N & T & MSEOLS & MSEDS\tabularnewline
\midrule
\endhead
2 & 10 & 1.8793 & 1.2295\tabularnewline
5 & 10 & 1.9473 & 0.7309\tabularnewline
10 & 10 & 1.9075 & 0.4363\tabularnewline
50 & 10 & 1.9488 & 0.2444\tabularnewline
2 & 20 & 0.4574 & 0.3079\tabularnewline
5 & 20 & 0.4475 & 0.2006\tabularnewline
10 & 20 & 0.4481 & 0.1643\tabularnewline
50 & 20 & 0.4557 & 0.1546\tabularnewline
2 & 50 & 0.1395 & 0.1140\tabularnewline
5 & 50 & 0.1395 & 0.1064\tabularnewline
10 & 50 & 0.1378 & 0.1136\tabularnewline
50 & 50 & 0.1389 & 0.1310\tabularnewline
%2 & 100 & 0.0636 & 0.0655\tabularnewline
%5 & 100 & 0.0638 & 0.0879\tabularnewline
%10 & 100 & 0.0644 & 0.1018\tabularnewline
%50 & 100 & 0.0643 & 0.1197\tabularnewline
\bottomrule
\end{longtable}
%\begin{longtable}[]{@{}llll@{}}
%\caption{Simulation Results Linear - out of sample - Setting 2, X iid,
%p=5}\tabularnewline
%\toprule
%N & T & MSEOLS & MSEDS\tabularnewline
%\midrule
%\endfirsthead
%\toprule
%N & T & MSEOLS & MSEDS\tabularnewline
%\midrule
%\endhead
%2 & 10 & 1.8793 & 1.2295\tabularnewline
%5 & 10 & 1.9473 & 0.7309\tabularnewline
%10 & 10 & 1.9075 & 0.4363\tabularnewline
%50 & 10 & 1.9488 & 0.2444\tabularnewline
%2 & 20 & 0.4574 & 0.3079\tabularnewline
%5 & 20 & 0.4475 & 0.2006\tabularnewline
%10 & 20 & 0.4481 & 0.1643\tabularnewline
%50 & 20 & 0.4557 & 0.1546\tabularnewline
%2 & 50 & 0.1395 & 0.1140\tabularnewline
%5 & 50 & 0.1395 & 0.1064\tabularnewline
%10 & 50 & 0.1378 & 0.1136\tabularnewline
%50 & 50 & 0.1389 & 0.1310\tabularnewline
%%2 & 100 & 0.0636 & 0.0655\tabularnewline
%%5 & 100 & 0.0638 & 0.0879\tabularnewline
%%10 & 100 & 0.0644 & 0.1018\tabularnewline
%%50 & 100 & 0.0643 & 0.1197\tabularnewline
%\bottomrule
%\end{longtable}
%\subsection{Lasso Setting}

==> sim_reg_mod.tex <==
\subsection{Regression Setting}
\begin{longtable}[htp]{@{}lllllll@{}}
	\caption{Simulation Results Linear - out of sample - Setting 1, X iid}\tabularnewline
	\toprule
	  &   &     & \multicolumn{2}{l}{p=5} & \multicolumn {2}{l}{p=10}  \tabularnewline
	N & T & cor & MSEOLS & MSEDS          & MSEOLS & MSEDS  \tabularnewline
	\midrule
	\endfirsthead
	\toprule
	  &   &     & \multicolumn{2}{l}{p=5} & \multicolumn {2}{l}{p=10}  \tabularnewline
	N & T & cor & MSEOLS & MSEDS          & MSEOLS & MSEDS  \tabularnewline
	\midrule
	\endhead
	2 & 10 & 0 & 2.0477 & 1.8037 & & \tabularnewline
	2 & 10 & 0.3 & 1.8083 & 1.5804& &\tabularnewline
	2 & 10 & 0.7 & 1.8056 & 1.3903& &\tabularnewline
	2 & 10 & 1 & 2.0681 & 1.1047& &\tabularnewline
	10 & 10 & 0 & 1.8735 & 1.3439& &\tabularnewline
	10 & 10 & 0.3 & 1.8975 & 1.2038& &\tabularnewline
	10 & 10 & 0.7 & 1.8734 & 0.8594& &\tabularnewline
	10 & 10 & 1 & 1.9841 & 0.2563& &\tabularnewline
	50 & 10 & 0 & 1.9364 & 1.6732& &\tabularnewline
	50 & 10 & 0.3 & 1.8925 & 1.5160& &\tabularnewline
	50 & 10 & 0.7 & 1.9256 & 0.9738& &\tabularnewline
	50 & 10 & 1 & 1.8750 & 0.0557& &\tabularnewline
	2 & 20 & 0 & 0.4585 & 0.4601 & 1.4150 & 1.3666\tabularnewline
	2 & 20 & 0.3 & 0.4429 & 0.4380 & 1.3444 & 1.2612\tabularnewline
	2 & 20 & 0.7 & 0.4405 & 0.4027 & 1.3695 & 1.1300\tabularnewline
	2 & 20 & 1 & 0.4509 & 0.2285 & 1.3662 & 0.6643 \tabularnewline
	10 & 20 & 0 & 0.4501 & 0.6132& 1.3668 & 1.1860 \tabularnewline
	10 & 20 & 0.3 & 0.4505 & 0.6299 & 1.3642 & 1.1461\tabularnewline
	10 & 20 & 0.7 & 0.4605 & 0.5729& 1.3681 & 0.9733\tabularnewline
	10 & 20 & 1 & 0.4546 & 0.0444 &1.3442 & 0.1208\tabularnewline
    50 & 20 & 0 && & 1.3651 & 1.6518\tabularnewline
    50 & 20 & 0.3 && & 1.3691 & 1.7681\tabularnewline
    50 & 20 & 0.7 && & 1.3730 & 1.4962\tabularnewline
    50 & 20 & 1 && & 1.3598 & 0.0211\tabularnewline
    2 & 50 & 0 && & 0.2896 & 0.2901\tabularnewline
    2 & 50 & 0.3 && & 0.2890 & 0.2890\tabularnewline
    2 & 50 & 0.7 && & 0.2942 & 0.3010\tabularnewline
    2 & 50 & 1 && & 0.2805 & 0.1429\tabularnewline
    10 & 50 & 0 && & 0.2907 & 0.3431\tabularnewline
    10 & 50 & 0.3 && & 0.2888 & 0.4161\tabularnewline
    10 & 50 & 0.7 && & 0.2856 & 0.5958\tabularnewline
    10 & 50 & 1 && & 0.2868 & 0.0270\tabularnewline
	\bottomrule
\end{longtable}


\begin{table}[!htb]
	\caption{Simulation Results Linear - out of sample - Setting 1, X cor,	p=5}\tabularnewline
\begin{minipage}{0.11\textwidth}
	\addtocounter{table}{-1}
\begin{longtable}[l]{@{}lllll@{}}
	\toprule
	N & T & cor & MSEOLS & MSEDS\tabularnewline
	\midrule
	\endfirsthead
	\toprule
	N & T & cor & MSEOLS & MSEDS\tabularnewline
	\midrule
	\endhead
	2 & 10 & 0 & 1.8411 & 1.6828\tabularnewline
	2 & 10 & 0.3 & 1.9002 & 1.6448\tabularnewline
	2 & 10 & 0.5 & 1.9717 & 1.6382\tabularnewline
	2 & 10 & 0.8 & 1.9106 & 1.4015\tabularnewline
	2 & 10 & 1 & 1.9148 & 1.1648\tabularnewline
	10 & 10 & 0 & 1.9718 & 1.4550\tabularnewline
	10 & 10 & 0.3 & 1.9239 & 1.2699\tabularnewline
	10 & 10 & 0.5 & 1.9413 & 1.1295\tabularnewline
	10 & 10 & 0.8 & 2.1294 & 0.9679\tabularnewline
	10 & 10 & 1 & 1.9357 & 0.3262\tabularnewline
	50 & 10 & 0 & 1.9365 & 1.6522\tabularnewline
	50 & 10 & 0.3 & 1.9011 & 1.4880\tabularnewline
	50 & 10 & 0.5 & 1.9335 & 1.2989\tabularnewline
	\bottomrule
\end{longtable}
\end{minipage}\qquad 
\begin{minipage}{0.7\textwidth}
	\addtocounter{table}{-1}
	\begin{longtable}[r]{@{}lllll@{}}
		\toprule
		N & T & cor & MSEOLS & MSEDS\tabularnewline
		\midrule
		\endfirsthead
		\toprule
		N & T & cor & MSEOLS & MSEDS\tabularnewline
		\midrule
		\endhead
	
		50 & 10 & 0.8 & 1.8970 & 0.7490\tabularnewline
		50 & 10 & 1 & 1.8919 & 0.0782\tabularnewline
		100 & 10 & 0 & 1.9235 & 1.9808\tabularnewline
		100 & 10 & 0.3 & 1.9332 & 1.7589\tabularnewline
		100 & 10 & 0.5 & 1.9416 & 1.4893\tabularnewline
		100 & 10 & 0.8 & 1.9211 & 0.8225\tabularnewline
		100 & 10 & 1 & 1.8920 & 0.0485\tabularnewline
		2 & 20 & 0 & 0.4459 & 0.4596\tabularnewline
		2 & 20 & 0.3 & 0.4490 & 0.4546\tabularnewline
		2 & 20 & 0.5 & 0.4526 & 0.4351\tabularnewline
		2 & 20 & 0.8 & 0.4789 & 0.4131\tabularnewline
		2 & 20 & 1 & 0.4717 & 0.2574\tabularnewline
		&&&&\\
		%10 & 20 & 0 & 0.4508 & 0.5969\tabularnewline
		%10 & 20 & 0.3 & 0.4466 & 0.6316\tabularnewline
		%10 & 20 & 0.5 & 0.4610 & 0.6230\tabularnewline
		%10 & 20 & 0.8 & 0.4475 & 0.4702\tabularnewline
		%10 & 20 & 1 & 0.4500 & 0.0497\tabularnewline
		\bottomrule
	\end{longtable}
\end{minipage}
\end{table}

\begin{table}[t]
\begin{longtable}[]{@{}llllll@{}}
	\caption{Simulation Results Linear - out of sample - Setting 2, p=5}\tabularnewline
	\toprule
	   &   & \multicolumn{2}{l}{X iid} & \multicolumn {2}{l}{X cor}  \tabularnewline
	 N & T & MSEOLS & MSEDS          & MSEOLS & MSEDS \tabularnewline
	\midrule
	\endfirsthead
	\toprule
  	  &       & \multicolumn{2}{l}{X idd} & \multicolumn {2}{l}{X cor}  \tabularnewline
	N & T     & MSEOLS & MSEDS          & MSEOLS & MSEDS  \tabularnewline
	\midrule
	\endhead
	2 & 10 & 1.7442 & 1.1173& 1.8793 & 1.2295\tabularnewline
	5 & 10 & 1.9357 & 0.6869& 1.9473 & 0.7309\tabularnewline
	10 & 10 & 1.9140 & 0.4323 & 1.9075 & 0.4363\tabularnewline
	50 & 10 & 1.9496 & 0.2680& 1.9488 & 0.2444\tabularnewline
	100 & 10 & 1.9326 & 0.2364&  & \tabularnewline
	2 & 20 & 0.4488 & 0.3057 & 0.4574 & 0.3079\tabularnewline
	5 & 20 & 0.4558 & 0.1996 &  0.4475 & 0.2006\tabularnewline
	10 & 20 & 0.4630 & 0.1653 & 0.4481 & 0.1643\tabularnewline
	50 & 20 & 0.4520 & 0.1561& 0.4557 & 0.1546\tabularnewline
	100 & 20 & 0.4544 & 0.1586&&\tabularnewline
	2 & 50 & 0.1416 & 0.1155& 0.1395 & 0.1140\tabularnewline
	5 & 50 & 0.1402 & 0.1071 & 0.1395 & 0.1064\tabularnewline
	10 & 50 & 0.1411 & 0.1160& 0.1378 & 0.1136\tabularnewline
	50 & 50 & 0.1375 & 0.1298& 0.1389 & 0.1310\tabularnewline
	100 & 50 & 0.1381 & 0.1336&&\tabularnewline
	2 & 100 & 0.0640 & 0.0663& 0.0636* & 0.0655*\tabularnewline
	\bottomrule
\end{longtable}
\end{table}
